Multivariate Physics-Informed Convolutional Autoencoder for Anomaly Detection in Power Distribution Systems with High Penetration of DERs

Despite the relentless progress of deep learning models in analyzing the system conditions under cyber-physical events, their abilities are limited in the power system domain due to data availability issues, cost of data acquisition, and lack of interpretation and extrapolation for the data beyond the training windows. In addition, the integration of distributed energy resources (DERs) such as wind and solar generations increases the complexities and nonlinear nature of power systems. Therefore, an interpretable and reliable methodology is of utmost need to increase the confidence of power system operators and their situational awareness for making reliable decisions. This has led to the development of physics-informed neural network (PINN) models as more interpretable, trustworthy, and robust models where the underlying principled laws are integrated into the training process of neural network models to achieve improved performance. This paper proposes a multivariate physics-informed convolutional autoencoder (PIConvAE) model to detect cyber anomalies in power distribution systems with unbalanced configurations and high penetration of DERs. The physical laws are integrated through a customized loss function that embeds the underlying Kirchhoff's circuit laws into the training process of the autoencoder. The performance of the multivariate PIConvAE model is evaluated on two unbalanced power distribution grids, IEEE 123-bus system and a real-world feeder in Riverside, CA. The results show the exceptional performance of the proposed method in detecting various cyber anomalies in both systems. In addition, the model's effectiveness is evaluated in data scarcity scenarios with different training data ratios. Finally, the model's performance is compared with existing machine learning models where the PIConvAE model surpasses other models with considerably higher detection metrics.

==> Refs_old.tex <==

@article{protocols,
  title={Review on cyber-physical and cyber-security system in smart grid: Standards, protocols, constraints, and recommendations},
  author={Hasan, M.K. and Habib, A.A. and Shukur, Z. and Ibrahim, F. and Islam, S. and Razzaque, M.A.},
  journal={Journal of Network and Computer Applications},
  volume={209},
  number={},
  pages={103540},
  year={Jan 2023. https://doi.org/10.1016/j.jnca.2022.103540}
  }

@article{cyber-physical,
  title={On the Cyber-Physical Needs of DER-based Voltage Control/Optimization Algorithms in Active Distribution Network},
  author={Majumder, S. and Vosughi, A. and Mustafa, H.M. and Warner, T.E. and Srivastava, A.K.},
  journal={IEEE Access},
  volume={},
  number={},
  pages={},
  year={May 2023. https://doi.org/10.1109/ACCESS.2023.3278281}
  }

@article{Dileep,
  title={ A survey on smart grid technologies and applications},
  author={Dileep, G},
  journal={Renewable energy},
  volume={146},
  number={},
  pages={2589-2625},
  year={Feb 2020. https://doi.org/10.1016/j.renene.2019.08.092}
  }

@article{sparsity_con,
  title={Stealth data injection attacks with sparsity constraints},
  author={Ye, X. and Esnaola, I. and Perlaza, S.M. and Harrison, R.F.},
  journal={IEEE Transactions on Smart Grid},
  volume={},
  number={},
  pages={},
  year={Jan 2023. https://doi.org/10.1109/TSG.2023.3238913}
  }

@article{multiple_dc,
  title={False data injection cyber-attacks detection for multiple DC microgrid clusters},
  author={Tan, S. and Xie, P. and Guerrero, J.M. and Vasquez, J.C.},
  journal={Applied Energy},
  volume={310},
  number={},
  pages={118425},
  year={Mar 2022. https://doi.org/10.1016/j.apenergy.2021.118425}
  }

@article{federated_learning,
  title={Incentive edge-based federated learning for false data injection attack detection on power grid state estimation: A novel mechanism design approach},
  author={Lin, W.T. and Chen, G. and Huang, Y.},
  journal={Applied Energy},
  volume={314},
  number={},
  pages={118828},
  year={May 2022. https://doi.org/10.1016/j.apenergy.2022.118828}
  }

@article{hybrid_DL,
  title={A hybrid deep learning model for discrimination of physical disturbance and cyber-attack detection in smart grid},
  author={Bitirgen, K. and Filik, Ü. B.},
  journal={International Journal of Critical Infrastructure Protection},
  volume={40},
  number={},
  pages={100582},
  year={Mar 2023}
  }

@article{critical_meter,
  title={Critical meter identification and network embedding based attack detection for power systems against false data injection attacks},
  author={Lian, X. and Qian, T. and Zhang, Y. and Tang, W. and Wu, Q.},
  journal={International Journal of Electrical Power & Energy Systems},
  volume={143},
  number={},
  pages={108389},
  year={Dec 2022}
  }

@article{DG_impact,
  title={Impact of distributed generation on protection and voltage regulation of distribution systems: A review},
  author={Razavi, S.E. and Rahimi, E. and Javadi, M.S. and Nezhad, A.E. and Lotfi, M. and Shafie-khah, M. and Catalão, J.P.},
  journal={Renewable and Sustainable Energy Reviews},
  volume={105},
  number={},
  pages={157-167},
  year={May 2019. https://doi.org/10.1016/j.rser.2019.01.050}
  }

@article{survey_physics,
  title={A survey of physics-based attack detection in cyber-physical systems},
  author={Giraldo, J. and Urbina, D. and Cardenas, A. and Valente, J. and Faisal, M. and Ruths, J. and Tippenhauer, N.O. and Sandberg, H. and Candell, R.},
  journal={ACM Computing Surveys (CSUR)},
  volume={51},
  number={4},
  pages={1-36},
  year={Jul 2018. https://doi.org/10.1145/3203245}
  }

@article{model_based_AGC,
  title={Model-based attack detection and mitigation for automatic generation control},
  author={Sridhar, S. and Govindarasu, M.},
  journal={IEEE Transactions on Smart Grid},
  volume={5},
  number={2},
  pages={580-591},
  year={Mar 2014. https://doi.org/10.1109/TSG.2014.2298195}
  }

@INPROCEEDINGS{HMM,
  author={Li, B., Lu, R. and Xiao, G.},
  booktitle={GLOBECOM 2017-2017 IEEE Global Communications Conference}, 
  title={HMM-based fast detection of false data injections in advanced metering infrastructure}, 
  year={Dec 2017. https://doi.org/10.1109/GLOCOM.2017.8254498},
  volume={},
  number={},
  pages={1-6}
  }

@article{PINN,
  title={Applications of physics-informed neural networks in power systems-a review},
  author={Huang, B. and Wang, J.},
  journal={IEEE Transactions on Power Systems},
  volume={38},
  number={1},
  pages={572-588},
  year={Mar 2022. https://doi.org/10.1109/TPWRS.2022.3162473}
  }

@article{PIML,
  title={Physics-Informed Machine Learning for Data Anomaly Detection, Classification, Localization, and Mitigation: A Review, Challenges, and Path Forward},
  author={Jabbari Zideh, M. and Chatterjee, P. and Srivastava, A. K.},
  journal={arXiv preprint arXiv:2309.10788},
  volume={},
  number={},
  pages={},
  year={2023. https://doi.org/10.48550/arXiv.2309.10788},
  doi = {}
  }


@article{reachability_FDIA,
  title={Reachability-based false data injection attacks and defence mechanisms for cyberpower system},
  author={Liu, R. and Mustafa, H.M. and Nie, Z. and Srivastava, A.K.},
  journal={Energies},
  volume={15},
  number={5},
  pages={1754},
  year={Feb 2022. https://doi.org/10.3390/en15051754}
  }

@article{NovelFDIA,
  title={A novel false data injection attack detection model of the cyber-physical power system},
  author={Cao, Jie and Da, Wang and Zhaoyang, Qu and Mingshi, Cui and Pengcheng, Xu and Kai, Xue and Kewei, Hu},
  journal={IEEE Access},
  volume={8},
  number={},
  pages={95109-95125},
  year={May 2020}
  }

@article{masking,
  title={Masking transmission line outages via false data injection attacks},
  author={Liu, Xuan and Zhiyi, Li and Xingdong, Liu and Zuyi, Li},
  journal={IEEE Transactions on Information Forensics and Security},
  volume={11},
  number={7},
  pages={1592-1602},
  year={Mar 2016. https://doi.org/10.1109/TIFS.2016.2542061}
  }

@article{survey_fdia,
  title={A survey on the detection algorithms for false data injection attacks in smart grids},
  author={Musleh, Ahmed S. and Guo, Chen and Zhao, Yang Dong},
  journal={IEEE Transactions on Smart Grid },
  volume={11},
  number={3},
  pages={2218-2234},
  year={Oct 2019. https://doi.org/10.1109/TSG.2019.2949998}
  }

@article{Data_Integrity,
  title={Data integrity attack detection using ensemble based learning for cyber physical power systems},
  author={Goyel, Himanshu and K. Shanti, Swarup},
  journal={IEEE Transactions on Smart Grid},
  volume={},
  number={},
  pages={},
  year={Aug 2022. https://doi.org/10.1109/TSG.2022.3199305}
  }

@article{realtime,
  title={Real-time detection of false data injection attacks in smart grid: A deep learning-based intelligent mechanism},
  author={He, Youbiao and Gihan, J. Mendis and Jin, Wei},
  journal={IEEE Transactions on Smart Grid},
  volume={8},
  number={5},
  pages={2505-2516},
  year={May 2017. https://doi.org/10.1109/TSG.2017.2703842}
  }

@article{scalable,
  title={A deep and scalable unsupervised machine learning system for cyber-attack detection in large-scale smart grids},
  author={Karimipour, H. and Dehghantanha, A. and Parizi, R.M. and Choo, K.K.R. and Leung, H},
  journal={IEEE Access},
  volume={7},
  number={},
  pages={80778-80788},
  year={May 2019. https://doi.org/10.1109/ACCESS.2019.2920326}
  }

@article{aligholian2021,
  title={Unsupervised event detection, clustering, and use case exposition in micro-pmu measurements},
  author={Aligholian, A. and Shahsavari, A. and Stewart, E.M. and Cortez, E. and Mohsenian-Rad, H.},
  journal={IEEE Transactions on Smart Grid},
  volume={12},
  number={4},
  pages={3624-3636},
  year={Mar 2021. https://doi.org/10.1109/TSG.2021.3063088}
  }

@article{transfer_hai,
  title={Transfer Learning for Event Detection From PMU Measurements With Scarce Labels},
  author={Hai, A.A. and Dokic, T. and Pavlovski, M. and Mohamed, T. and Saranovic, D. and Alqudah, M. and Kezunovic, M. and Obradovic, Z.},
  journal={IEEE Access},
  volume={9},
  number={},
  pages={127420-127432},
  year={Sep 2021. https://doi.org/10.1109/ACCESS.2021.3111727
}
  }

@INPROCEEDINGS{radial_ring,
  author={Deyhimi, N. and Torkaman, H. and Shadaei, M. and Shabanirad, M. and Kermani, M.},
  booktitle={2021 IEEE International Conference on Environment and Electrical Engineering and 2021 IEEE Industrial and Commercial Power Systems Europe (EEEIC/I&CPS Europe) }, 
  title={Comparative Multi-objective Investigation of Radial and Ring Distribution System in the Presence of DGs}, 
  year={Sep 2021. https://doi.org/10.1109/EEEIC/ICPSEurope51590.2021.9584527},
  volume={},
  number={},
  pages={1-6}
  }

@article{AD_building,
  title={Analytical investigation of autoencoder-based methods for unsupervised anomaly detection in building energy data},
  author={Fan, C. and Xiao, F. and Zhao, Y. and Wang, J.},
  journal={Applied Energy},
  volume={211},
  number={},
  pages={1123-1135},
  year={Feb 2018. https://doi.org/10.1016/j.apenergy.2017.12.005}
  }

@article{fast_ramped,
  title={Unsupervised detection and open-set classification of fast-ramped flexibility activation events},
  author={Müller, N. and Heinrich, C. and Heussen, K. and Bindner, H.W.},
  journal={Applied Energy},
  volume={312},
  number={},
  pages={118647},
  year={Apr 2022. https://doi.org/10.1016/j.apenergy.2022.118647}
  }

@article{solar_farm,
  title={Solar farm voltage anomaly detection using high-resolution μPMU data-driven unsupervised machine learning},
  author={Dey, M. and Rana, S.P. and Simmons, C.V. and Dudley, S.},
  journal={Applied Energy},
  volume={303},
  number={},
  pages={117656},
  year={Dec 2021. https://doi.org/10.1016/j.apenergy.2021.117656}
  }

@INPROCEEDINGS{aligholian2020,
  author={Aligholian, A. and Shahsavari, A. and Cortez, E. and Stewart, E. and Mohsenian-Rad, H.},
  booktitle={2020 IEEE Power & Energy Society General Meeting (PESGM)}, 
  title={Event detection in micro-pmu data: A generative adversarial network scoring method}, 
  year={Aug 2020. https://doi.org/10.1109/PESGM41954.2020.9281560},
  volume={},
  number={},
  pages={1-5}
  }

@INPROCEEDINGS{david2020,
  author={Amoateng, D.O. and Yan, R. and Saha, T.K.},
  booktitle={2020 IEEE Power & Energy Society General Meeting (PESGM)}, 
  title={A deep unsupervised learning approach to PMU event detection in an active distribution network}, 
  year={Aug 2020. https://doi.org/10.1109/PESGM41954.2020.9281767},
  volume={},
  number={},
  pages={1-5}
  }

@INPROCEEDINGS{naderi2022,
  author={Naderi, E. and Aydeger, A. and Asrari, A.},
  booktitle={2022 IEEE Conference on Technologies for Sustainability (SusTech)}, 
  title={Detection of false data injection cyberattacks targeting smart transmission/distribution networks}, 
  year={Apr 2022. https://doi.org/10.1109/SusTech53338.2022.9794237},
  volume={},
  number={},
  pages={224-229}
  }

@article{semi-Supervised,
  title={Detecting false data injection attacks in smart grids: A semi-supervised deep learning approach},
  author={Zhang, Ying and Jianhui, Wang and Bo, Chen},
  journal={IEEE Transactions on Smart Grid},
  volume={12},
  number={1},
  pages={623-634},
  year={Jul 2020. https://doi.org/10.1109/TSG.2020.3010510}
  }

@article{hierarchical,
  title={Adaptive hierarchical cyber attack detection and localization in active distribution systems},
  author={Li, Qi and Jinan, Zhang and Junbo, Zhao and Jin, Ye and Wenzhan, Song and Fangyu, Li},
  journal={IEEE transactions on smart grid},
  volume={13},
  number={3},
  pages={2369-2380},
  year={Feb 2022. https://doi.org/10.1109/TSG.2022.3148233}
  }

  @article{islanded_MG,
  title={Data-driven cyber-attack detection of intelligent attacks in islanded dc microgrids},
  author={Wan, Yihao and Tomislav, Dragičević},
  journal={IEEE Transactions on Industrial Electronics},
  volume={70},
  number={4},
  pages={4293-4299},
  year={May 2022. https://doi.org/10.1109/TIE.2022.3176301}
  }

  @article{volt_reg,
  title={Detection of cyber attacks on voltage regulation in distribution systems using machine learning},
  author={Bhusal, Narayan and Mukesh, Gautam and Mohammed, Benidris},
  journal={IEEE Access},
  volume={9},
  number={},
  pages={40402-40416},
  year={Mar 2021. https://doi.org/10.1109/ACCESS.2021.3064689}
  }

@article{NARX,
  title={Detection of false data injection cyber-attacks in DC microgrids based on recurrent neural networks},
  author={Habibi, M. R. and Baghaee, H. R. and Dragičević, T. and Blaabjerg, F.},
  journal={IEEE Journal of Emerging and Selected Topics in Power Electronics},
  volume={9},
  number={5},
  pages={5294-5310},
  year={Jan 2020. https://doi.org/10.1109/JESTPE.2020.2968243}
  }

@article{coordinated,
  title={Coordinated data falsification attack detection in the domain of distributed generation using deep learning},
  author={Bhusal, N. and Gautam, M. and Shukla, R.M. and Benidris, M. and Sengupta, S.},
  journal={International Journal of Electrical Power & Energy Systems},
  volume={134},
  number={},
  pages={107345},
  year={Jan 2022. https://doi.org/10.1016/j.ijepes.2021.107345}
  }

@article{raghuvamsi,
  title={Detection and reconstruction of measurements against false data injection and DoS attacks in distribution system state estimation: A deep learning approach},
  author={Raghuvamsi, Y. and Teeparthi, K.},
  journal={Measurement},
  volume={210},
  number={},
  pages={112565},
  year={Mar 2023. https://doi.org/10.1016/j.measurement.2023.112565}
  }

@article{radhoush2023,
  title={Distribution System State Estimation and False Data Injection Attack Detection with a Multi-Output Deep Neural Network},
  author={Radhoush, S. and Vannoy, T. and Liyanage, K. and Whitaker, B.M. and Nehrir, H.},
  journal={Energies},
  volume={16},
  number={5},
  pages={2288},
  year={Feb 2023. https://doi.org/10.3390/en16052288}
  }

@INPROCEEDINGS{TadGAN,
  author={Geiger, A. and Liu, D. and Alnegheimish, S. and Cuesta-Infante, A. and Veeramachaneni, K.},
  booktitle={2020 IEEE International Conference on Big Data (Big Data)}, 
  title={Tadgan: Time series anomaly detection using generative adversarial networks}, 
  year={Dec 2020. https://doi.org/10.1109/BigData50022.2020.9378139},
  volume={},
  number={},
  pages={33-43}
  }


@article{bhanja,
  title={Impact of data normalization on deep neural network for time series forecasting},
  author={Bhanja, S. and Das, A.},
  journal={arXiv preprint arXiv:1812.05519},
  volume={},
  number={},
  pages={},
  year={Dec 2018. https://doi.org/10.48550/arXiv.1812.05519}
  }

@article{jayala,
  title={Statistical normalization and back propagation for classification},
  author={Jayalakshmi, T. and Santhakumaran, A.},
  journal={International Journal of Computer Theory and Engineering},
  volume={3},
  number={1},
  pages={1793-8201},
  year={Feb 2011. https://doi.org/10.7763/IJCTE.2011.V3.288}
  }

@article{stock_idex,
  title={Impact of data normalization on stock index forecasting},
  author={Nayak, S.C. and Misra, B.B. and Behera, H.S.},
  journal={International Journal of Computer Information Systems and Industrial Management Applications},
  volume={6},
  number={2014},
  pages={257-269},
  year={Jan 2014}
  }

@INPROCEEDINGS{solar_irad,
  author={Nematirad, R. and Pahwa, A.},
  booktitle={2022 IEEE Kansas Power and Energy Conference (KPEC)}, 
  title={Solar radiation forecasting using artificial neural networks considering feature selection}, 
  year={Apr 2022. https://doi.org/10.1109/KPEC54747.2022.9814765},
  volume={},
  number={},
  pages={1-4}
  }

@article{sliding_window,
  title={Online fault monitoring based on deep neural network & sliding window technique},
  author={Saeed, H.A. and Wang, H. and Peng, M. and Hussain, A. and Nawaz, A.},
  journal={Progress in Nuclear Energy},
  volume={121},
  number={},
  pages={103236},
  year={Mar 2020. https://doi.org/10.1016/j.pnucene.2019.103236}
  }

@INPROCEEDINGS{autoencoder_AD,
  author={Sakurada, M. and Yairi, T.},
  booktitle={2Proceedings of the MLSDA 2014 2nd workshop on machine learning for sensory data analysis}, 
  title={Anomaly detection using autoencoders with nonlinear dimensionality reduction}, 
  year={Dec 2014. http://dx.doi.org/10.1145/2689746.2689747},
  volume={},
  number={},
  pages={4-11}
  }

@article{GAN,
  title={Generative adversarial networks},
  author={Goodfellow, I. and Pouget-Abadie, J. and Mirza, M. and Xu, B. and Warde-Farley, D. and Ozair, S. and Courville, A. and Bengio, Y.},
  journal={arXiv preprint arXiv:1406.2661},
  volume={},
  number={},
  pages={},
  year={2014. 
https://doi.org/10.48550/arXiv.1406.2661}
  }
  @INPROCEEDINGS{WGAN,
  author={Arjovsky, M. and Chintala, S. and Bottou, L.},
  booktitle={International conference on machine learning}, 
  title={Wasserstein generative adversarial networks}, 
  year={PMLR, Jul 2017},
  volume={},
  number={},
  pages={214-223}
  }

  @INPROCEEDINGS{camouflage,
  author={Bhattacharjee, S. and Thakur, A. and Das, S.K.},
  booktitle={Proceedings of the 2018 on Asia Conference on Computer and Communications Security}, 
  title={Towards fast and semi-supervised identification of smart meters launching data falsification attacks}, 
  year={May 2018. https://doi.org/10.1145/3196494.3196551},
  volume={},
  number={},
  pages={173-185}
  }

@article{iterative,
  title={An Iterative Method for Detection of the Collusive Strategy in Prisoner’s
Dilemma Game of Electricity Market},
  author={Mohtavipour, Seyed Saeid and Jabbari Zideh, M.},
  journal={EEJ Transactions on Electrical and Electronic Engineering},
  volume={14},
  number={2},
  pages={252-260},
  year={Feb 2019. https://doi.org/10.1002/tee.22804}
  }

@article{NREL,
  title={},
  author={},
  journal={},
  volume={},
  number={},
  pages={},
  year={“Weather Data,” National Renewable Energy Laboratory, [Online]. Available: https://sam.nrel.gov/weather-data.html. [Accessed 5 Dec 2022].}
  }

  @INPROCEEDINGS{DTW,
  author={Berndt, D.J. and Clifford, J.},
  booktitle={KDD workshop}, 
  title={Using dynamic time warping to find patterns in time series}, 
  year={Jul 1994},
  volume={},
  number={},
  pages={359-370}
  }

@INPROCEEDINGS{gradient,
  author={Gulrajani, I. and Ahmed, F. and Arjovsky, M. and Dumoulin, V. and Courville, A.C.},
  booktitle={Proc. of the 31st Int. Conf. on Neural Information
Processing Systems}, 
  title={Improved Training of Wasserstein GANs}, 
  year={2017},
  volume={},
  number={},
  pages={5769–5779}
  }

  @article{test_systems,
  title={IEEE PES Distribution Systems Analysis Subcommittee Radial Test Feeders. [Online]. Available: https://cmte.ieee.org/pes-testfeeders/resources/. Accessed: Sep 2023},
  author={},
  journal={},
  year={}
}


  @article{turbulence,
  title={A physics-aware machine to predict extreme events in turbulence},
  author={Doan, N.A.K. and Polifke, W. and Magri, L.},
  journal={arXiv preprint},
  year={2019}
}

@book{suttonbartorl,
author = {Sutton, R. and Barto, A.},
title = {Reinforcement {L}earning: {A}n {I}ntroduction},
publisher = {The MIT Press},
address = {Cambridge MA},
year = {2018}
}

@INPROCEEDINGS{RL_PCC,
  author={Wang, Xinming and Liu, Haotian and Cao, Xin and Wu, Wenchuan and Li, Shihui and Jia, Xiaobu},
  booktitle={2021 Power System and Green Energy Conference (PSGEC)}, 
  title={Active and Reactive Power Coordinated Control of Active Distribution Networks Based on Prioritized Reinforcement Learning}, 
  year={2021. https://doi.org/10.1109/PSGEC51302.2021.9541702},
  volume={},
  number={},
  pages={91-96},
  }
